Distributed Collaborative Monitoring in Software Defined Networks

We propose a Distributed and Collaborative Monitoring system, DCM, with the following properties. First, DCM allow switches to collaboratively achieve flow monitoring tasks and balance measurement load. Second, DCM is able to perform per-flow monitoring, by which different groups of flows are monitored using different actions. Third, DCM is a memory-efficient solution for switch data plane and guarantees system scalability. DCM uses a novel two-stage Bloom filters to represent monitoring rules using small memory space. It utilizes the centralized SDN control to install, update, and reconstruct the two-stage Bloom filters in the switch data plane. We study how DCM performs two representative monitoring tasks, namely flow size counting and packet sampling, and evaluate its performance. Experiments using real data center and ISP traffic data on real network topologies show that DCM achieves highest measurement accuracy among existing solutions given the same memory budget of switches.

==> draft.tex <==




\section{System design}
The goal of DCM is to provide a scheme of 
network measurement, in which the \textit{per-flow} network traffic 
can be measured \textit{jointly} by multiple routers.

In this section, we give a detailed introduction to XXX. 
First , we explain how bloom filter is applied to make such 
monitoring can be done in a distributively way.
Then we show how to carry out packet level sampling with 
given sampling ratio for each flow.


\subsection{Model}

In our discussion , we use these following notations.
\begin{itemize}
\item $F_1,F_2, \cdots F_n$ are the flows that needed to be monitored 
in the network. 
\item $S=\{S_1,S_2, \cdots ,S_m\}$ are the switches in the network.
\item $P_{ij}$ is the $j$-th switch on flow $F_i$'s path. Such routing information 
is known to the coordinator. 
\end{itemize}

\subsubsection{Decision Bloom Filter: Pick out my flows}
A decision bloom filter is a bloom filter of flows.
Each switch $S_k$ holds a bloom filter $BF$-$Decision(S_k)$, by which the switch
decides whether a flow that goes through should be monitored. For every flow $F_i$,
at least one of such \textbf{Decision Bloom Filters} on the path of this flow, i.e.,
$BF$-$Decision(P_{ij})$ contains $F_i$.
Figure \ref{fig:ex1} shows a simple network. $BF$-$Decision(S_2)$ = $\{F_1\}$,
$BF$-$Decision(S_3)$=$\{F_2,F_3\}$.

The accuracy of many network monitoring applications have strong connections with 
the measurement load on it. For example, a count-minimum sketch will demonstrate 
lower accuracy  when it processes too many different flows. By distributing the measurement
load we may achieve a better accuracy. Moreover, the CPU ability on a switch 
also limits the number of different flows that processes.
Hence , for each bloom filter $S_k$, we define a 
threshold as $maxload(S_k)$, which indicates the maximum number of different flows
that can be processed by $S_k$.

We provide an algorithm described as \textbf{BalanceAllocate}. \textbf{BalanceAllocate} assigns flows to switches,
it balances the work load among switches and using a minimum number of different switches.
In the algorithm , only $avaliable$ switches are utilized for monitoring. Note that the CPU/Memory resource 
is necessary only if one switch is considered available.
When there is a new flow $F_i$ to be monitored, the algorithm first try to find a existing available switch on 
its path that is not over loaded. If such switch does not exist, a new switch is marked as available. 
In some extreme cases, all of the switch on its path are overloaded, the algorithm will pick the one with the relatively 
minimal load.


\begin{codebox}
\Procname{\proc{ \textbf{BalanceAllocate($BF$-$Decision$)}}}
\textbf{input}: Bloom Filters $BF$-$Decision$ and flows $F_1,F_2,...$.\\
\li Clear all $BF$-$Decision(S_k)$
\li For all $S_k$, let $Avaliable(S_k) $ = $False$
\li \While there is a new flow $F_i$ to be monitored 
\li \Do   $S_\alpha$=Find $P_{ij}$ with the smallest $BF$-$Decision(P_{ij})$ \\
 \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ that $Avaliable(P_{ij})= True$ \\
\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ and $size(BF\text{-}Decision(P_{ij})) < maxload(P_{ij})$
\li \If $S_\alpha$ does not exist
\li \Then \If there is at least one $P_{ij}$ that $Avaliable(P_{ij}) = False$
\li \Then $S_\alpha$ = randomly pick up one $P_{ij}$ that $Avaliable(P_{ij})=False$
          $Avaliable(S_\alpha) = True$
\li \Else $S_\alpha$=Find $P_{ij}$ with smallest $BF$-$Decision(P_{ij})$
 \End \End \End
\li Insert $F_i$ to $BF$-$Decision(S_\alpha)$
              \End

\end{codebox}





\subsubsection{Col. hash-based sampling}
To get a sample subset of a set of objects with a given ratio $p$, one possible approach
is to derive a hash value in $[0,1)$ for each object with a global hash function $H$, and take the ones with 
hash value less than $p$ as a sample subset. Consider $l$ positive values,
$0 < p_i <1 $ and $p_1+p_2+\cdots+ p_l= p$, and $l$ disjoint intervals in $[0,1)$:
$I_1=[x_1,x_1+p_1)$,$I_2=[x_2,x_2+p_2)$,$\cdots$,$I_l=[x_l,x_l+p_l)$.

For a given packet $M$ , which will be processed on $l$ switches on its path, one after another. It's intuitively 
to assign switches with interval $I_1,I_2,\cdots,I_l$ to each of them.
A packet is considered to be positively sampled as long as its hash value falls in 
one of the intervals.
In such way , switches can \textit{jointly} sample a given flow with rate $p$.

For a given ratio $p$, we can easily find the binary expression of $p$, and construct a corresponding number sequence ${p_l}$. Let the $b_i$ be the position of the $i$-th $1$ in $p$'s binary expression. For example , for $\frac{11}{16} = 
(0.1011)_2$, $b_1 = 1, b_2 = 3, b_3 = 4$, since the first, third and fourth position of the binary expression is 1.
$$p = \sum_{i=1}^{\infty} 2^{-b_i}$$

We can construct disjoint intervals of length $2^{-t}$, where $t$ is any positive integer. These intervals are:
$B_1=[\frac{1}{2},1)$,$B_2=\frac{1}{4},\frac{1}{2})$,$B_3=[\frac{1}{8},\frac{1}{4})$,$\cdots$,$B_t= [2^{-t},2^{-t+1})$.
For a given ratio $p$, derive the corresponding $b_i$ series from $p$'s binary expression.



\subsection{Balanced Joint Sampling}

Taking advantage of bloom filter and joint hash-based sampling, we can distribute the sampling workload among
switches.
For a given flow $F_i$ with required sampling rate $p$, the corresponding disjoint intervals $B_{b_1},B_{b_2},\cdots$ 
can be assigned to multiple switches on $F_i$'s path. Simultaneously, since all switch in 
such network share a same set of intervals, a switch can memorize the interval-flow combinations that assigned
to itself. Such work can be done with bloom filters. 

The process of assigning intervals goes similar to \textbf{BalanceAllocate}, which is described as below.
Every switch in the network keeps multiple bloom filters $BF_1$,$BF_2$,$\cdots$. $BF_i$ represents the 
set of all flows that is assigned with interval $B_i$ on this switch.


 

\begin{codebox}
\Procname{\proc{ \textbf{ALGO2}}}
\textbf{input}: flows $F_1,F_2,...$ and ratios $p_1,p_2,\cdots$\\
\li Clear all $BF_i(S_k)$
\li For all $S_k$, let $Avaliable_t(S_k) $ = $False$
\li \While there is a new flow $F_i$ to be monitored with ratio $r_i$
\li \Do calculate the binary expression of $r_i$
\li     calculate $b_1,b_2,\cdots$ for $r_i$.
\li     \For each $b_t$ 
\li     \Do
\li          $S_\alpha$=pick up $R_{ij}$ among all available and not-overloaded switches with smallest $B_t$
\li          Insert $F_i$ into $B_t(S_\alpha)$.
\li 
\end{codebox}
\subsection{Full Overview of the Architecture }
\begin{itemize}
\item wild-card
\item Decision
\item Rate
\end{itemize}
\subsubsection{what does a switch do when receive a packet}
\begin{itemize}
\item calculate $H_{wildcard}(x.flowInfo)$ ... if pass
\item calculate H(x)
\item decide $t$ that $B_t$ contains $H(x)$
\item if $x.flow$ in $BF_t$, report
\end{itemize}
\subsection{False positive analysis}



\subsection{Disscussion of Implementation}
component has already implemented in opensketch.
bf can be stored in tcam.


\section{Case Study (Evaluation) }
\subsection{Evaluation Settings}
data,
competitive algorithms:
aggregation rules
\subsection{Filter memory ratio}

Fig \ref{fig:ratio} shows the overestimate ratio. Total memory used = 1M / switch.
 \begin{figure}[t]
 \center
 \includegraphics[width=0.85\linewidth]{gra/graph1.eps}
 \caption{examp}
 \label{fig:ratio}
 \end{figure}
       



\subsection{Counting sketch}
count-min sketch accuracy . \\
lines: all at all, all at one, aggregation. \\
x:    total memory consumption \\
y:    relative error ( false positive ) , average 

\begin{figure*}[t!]
\centering

\begin{subfigure}[b]{0.3\textwidth}
\includegraphics[width=\linewidth]{gra/graph2unv1.eps}\caption{EDU1}
\label{fig:CntDcCaida}
\end{subfigure}
\begin{subfigure}[b]{0.3\textwidth}
\includegraphics[width=\linewidth]{gra/graph2fattree.eps}\caption{Fat Tree}
\label{fig:CntDcFT}
\end{subfigure}
\begin{subfigure}[b]{0.3\textwidth}
\includegraphics[width=\linewidth]{gra/graph2rocket.eps}\caption{Rocketfuel}
\label{fig:CntDcRo}
\end{subfigure}
\caption{CountMin Sketch: Data Center Trace}
\end{figure*}




\begin{figure*}[t]
\centering
\begin{subfigure}[b]{0.3\textwidth}
\includegraphics[width=\linewidth]{gra/graph2unv1Caida.eps}\caption{EDU1}
\label{fig:CntDcCaida}
\end{subfigure}
\begin{subfigure}[b]{0.3\textwidth}
\includegraphics[width=\linewidth]{gra/graph2fattreeCaida.eps}\caption{Fat Tree}
\label{fig:CntDcFT}
\end{subfigure}
\begin{subfigure}[b]{0.3\textwidth}
\includegraphics[width=\linewidth]{gra/graph2rocketCaida.eps}\caption{Rocketfuel}
\label{fig:CntDcRo}
\end{subfigure}
\caption{CountMin Sketch: ISP Trace}
\end{figure*}





\begin{figure*}[t]
\centering

\begin{subfigure}[b]{0.3\textwidth}
\includegraphics[width=\linewidth]{gra/graph3eduunv1.eps}\caption{EDU}
\label{fig:CntDcCaida}
\end{subfigure}
\begin{subfigure}[b]{0.3\textwidth}
\includegraphics[width=\linewidth]{gra/graph3eduft.eps}\caption{Fat Tree}
\label{fig:CntDcFT}
\end{subfigure}
\begin{subfigure}[b]{0.3\textwidth}
\includegraphics[width=\linewidth]{gra/graph3edurocket.eps}\caption{Rocketfuel}
\label{fig:CntDcRo}
\end{subfigure}
\caption{Sample: Data Center Trace}
\end{figure*}


\begin{figure*}[t]
\centering
\begin{subfigure}[b]{0.3\textwidth}
\includegraphics[width=\linewidth]{gra/graph3caidaunv1.eps}\caption{EDU1}
\label{fig:CntDcCaida}
\end{subfigure}
\begin{subfigure}[b]{0.3\textwidth}
\includegraphics[width=\linewidth]{gra/graph3caidaft.eps}\caption{Fat Tree}
\label{fig:CntDcFT}
\end{subfigure}
\begin{subfigure}[b]{0.3\textwidth}
\includegraphics[width=\linewidth]{gra/graph3caidarocket.eps}\caption{Rocketfuel}
\label{fig:CntDcRo}
\end{subfigure}
\caption{Sample: ISP Trace}
\end{figure*}






\begin{figure}
\includegraphics[width=0.85\linewidth]{gra/ratesCaidaFt.eps}\caption{Caida Fattree}
\end{figure}
\begin{figure}
\includegraphics[width=0.85\linewidth]{gra/ratesEduUnv.eps}\caption{Edu Unv}
\end{figure}
\subsection{Sampling}
sample accuracy\\
lines: distributed, (modified) aggregation. \\
x: total memory consumption \\
y: false positive sample

\section{Discussion and Future work}
\subsection{Dynamic Allocation}
\subsection{Re-construction of BF with few false positives}

\section{Conclusion}



==> future-old.tex <==
\section{Discussion and Future Work}

In dynamic networking settings, the flow set that people want to monitor 
and measure may change over time. In our current work, we does not discuss 
how to update the Bloom Filters when interested flow set changes. 
Using Counting Bloom Filter\cite{summarycache}, people can insert or 
delete elements in the set incrementally with modest overhead. 
In our future work, we would like to develop a lightweight 
but efficient method to dynamically update the Bloom Filters, 
with the aid of Counting Bloom Filter.

%False positive in Bloom Filter is not desired in our system. 
The accuracy of Bloom Filter could be further improved if false 
positive can be detected. If the central controller detects duplication, 
reconstructing the corresponding Bloom Filter that cause the duplication 
could eliminate this particular false positive and hence improving the accuracy.
 One possible way is cascading a table after the Bloom Filter to 
 record the queries that case false positive. 
 A flow is sampled only when it passes the Bloom Filter 
 and it is not in the following table. 
 We plan to test the feasibility of such method and measure the improvement in a quantitative way.  
 
 
% \subsection{}

%wild card rule is used to process flows that can be easily agggregated.....


%bloom filter length growth.



%.....false positive re-construction.



%memory is good, what about other resources? 



==> rel.tex <==

\subsection{Related works}
Network measurement and analysis are the concern for networking community for a long time.
 Packet-based sampling measurement methods, such as Netflow\cite{Netflow}
 and sFlow\cite{sflow} were proposed. Further, Authors in \cite{revisiting}
 state the importance of using per flow monitoring. cSamp\cite{csamp}, one per flow monitoring,
 utilizes hash-function to coordinate network-wide routers to
eliminate duplicate measurement in the network.
 A omniscient central controller which knows the flow path is needed.

 In recent years, there are a number of other monitor methods based on SDN, such as OpenSketch\cite{opensketch},
   a sketch-based sampling proposal.
    The resource of SDN switch is limited. Only limited number of rules can be store
    on SDN switch\cite{DIFANE}. Solutions like \cite{payless} and \cite{AggregationYinZhang} aggregate the rules to save the resource,
     \cite{palette} decompose rules into different tables and distribute on different switches.
     \cite{moshref2013resource} discusses the tradeoff between the resource and accuracy of the sampling.
      Decor\cite{Decor} finds a way to use local information to avoid the use of central controller to reinforce the robustness.

%Payless's related work is really good and detailed.

%Opensketch\cite{opensketch}->sketch-based sample, programmable measurement, hash-based, software-defined measurement
%cSamp\cite{csamp}-> flow sample, hash-based coordination, OD pairs
%Palette\cite{palette}->distributed table, reduce rule number.
%NetFlow\cite{Netflow}, sFlow\cite{sflow}->sample-based measurement
%Tradeoff\cite{Tradeoff}-> resource, primitives
%openTM\cite{openTM}->distributed query
%daptive Flow Counting\cite{Aggregation}-> aggregation to reduce rule number
%Decor\cite{Decor}->distributed decision making
%Payless\cite{payless}->statistics collection at different aggregation level
%DIFANE\cite{DIFANE}-> reduce the press of central controller
%revisiting\cite{revisiting}-> the importance of network flow monitoring
%cSamp-T\cite{cSamp-T}->without OD pairs.
%ProgME\cite{ProgME}->flowset




